Minority Voter Distributions and Partisan Gerrymandering

Many people believe that it is disadvantageous for members aligning with a minority party to cluster in cities, as this makes it easier for the majority party to gerrymander district boundaries to diminish the representation of the minority. We examine this effect by exhaustively computing the average representation for every possible $5\times 5$ grid of population placement and district boundaries. We show that, in fact, it is advantageous for the minority to arrange themselves in clusters, as it is positively correlated with representation. We extend this result to more general cases by considering the dual graph of districts, and we also propose and analyze metaheuristic algorithms that allow us to find strong lower bounds for maximum expected representation.

==> sections/clustering.tex <==
%\label{sec:clustering-relation}
%\begin{Conj}
%\label{conj:clustering-relation}
%	\textbf{(Clustering Relation).} For minority $\mathsf{NumH}$, there is a positive correlation between $\mathsf{ClusH}$ and $\mathbb{E}(\mathsf{Rep}_\Delta)$. 
%\end{Conj}
%
%
%	\begin{Def}
%	The \emph{discrete $n$-neighborhood} $N_n(b_i)$ of a $b_i\in V$ of our dual graph $G=(V,E)$ is the set of all blocks $b_j$ in $V$ such that there is a chain of at most $n$ edges that connect it to $b_u$. 
%	\begin{equation}
%		N_n(b_i) = \{b_j\in V\ |\ \exists \text{ path } p\subseteq E\text{ s.t. }\#p<n\}.
%	\end{equation}
%	For $n=0$, we say $N_0(b_i)=\{b_i\}$ is the set containing only $b_i$. 
%	\end{Def}
%	
%	\begin{Def}
%	The \emph{$n$-ring neighborhood} $R_n(b_i)$ is the set of all points in the $n$-neighborhood of $b_i$ but not in the $(n-1)$-neighborhood of $b_i$. 
%	\begin{equation}
%		R_n(b_i) = \{b_j\in N_n(b_i)\ |\ b_j\not\in N_{n-1}(b_i)\}
%	\end{equation}
%	\end{Def}
%	
%	\begin{Def}
%	$p_k(n)$ is the probability that a district of size $k$ (or $k$-omino) drawn to contain $b_i$ contains a block in the $n$-ring neighborhood of $b_i$. 
%	\end{Def}
%	
%	\begin{Rem}
%	\label{rem:adjacent-block}
%	For $k\geq 2, p_k(1) = 1$ as some block adjacent to $b_i$ has to be in a nontrivial district containing $b_i$. 
%	\end{Rem}
%	
%	\begin{Lemma}
%	\label{lemma:clustering}
%		For all $n$, 
%		\begin{equation}
%			p_k(n) \geq p_k(n+1)
%		\end{equation}
%	\end{Lemma}
%	\begin{proof} (of Lemma \ref{lemma:clustering})
%	We prove by induction on $n$. 
%	
%	\noindent If $k=1$, $p_k(n) = 0,\ \forall\ n>1$, so we are done. Otherwise consider $k\geq 2$. 
%	
%	\noindent \textbf{Base case:} $p_k(1)=1\geq p_k(2)$ by Remark \ref{rem:adjacent-block}.
%	
%	\noindent \textbf{Inductive step:} We assume that $p_k(m)\geq p_k(m+1)$ for all $m<n$. Let $b_n\in R_n(b_i)$ and $b_{n+1}\in R_{(n+1)}(b_i)$ be some blocks in their corresponding ring neighborhoods. 
%	\begin{align*}
%		p_k(n) &= P(\exists b_n\in d) \\
%		&= P(\exists b_n\in d\ \land\ \exists b_{n+1}\in d) + P(\exists b_n\in d\ \land\not\exists b_{n+1}\in d)
%		\intertext{Note that if a $n+1$ block is in our district, then the edge path it traces out includes an $n$ block, so an $n$ block must also be in our district. So}
%		&= P(\exists b_{n+1}\in d) + P(\exists b_n\in d\ \land\not\exists b_{n+1}\in d)\\
%		&= p_k(n+1) + P(\exists b_n\in d\ \land\not\exists b_{n+1}\in d).
%	\end{align*}
%	As $P(\exists b_n\in d\land\not\exists b_{n+1}\in d) \geq 0$, then $p_k(n) \geq p_k(n+1)$. This completes our proof. 
%	\end{proof}
%	
%	\begin{Rem}
%	\label{rem:diminishing-values}
%		At the point where $k < |N_n(b_i)|$, there becomes $k$-omino tilings wholly within $N_n(b_i)$, so $P(\exists b_n\in d\ \land\not\exists b_{n+1}\in d) > 0$ becomes strictly greater. Additionally, we note that $n > k$, $p_k(n) = 0$, as no district can span a distance of more blocks in itself. We can conclude that $p_k(n)$ tends to $0$ as $n$ tends to $k$. 
%	\end{Rem}
%	
%	\begin{proof} (of Conjecture \ref{conj:clustering-relation})
%	Note that the probability that \emph{some} given block being in a winning district is positively correlated to the expected outcome over the entire graph. We can thus find the general relation between clustering and the expected outcome of a given district containing block $b_i$. Let district $d$ contain an arbitrary block $b_i$ (where $\Delta(b_i) = 1$) and have $k$ total blocks. We can approximate the expected proportion of voters voting for a given party in district $d$, $\frac{1}{k}\mathbb{E}\left(\Delta_d\right)$:
%	\begin{align*}
%		\frac{1}{k}\mathbb{E}(\Delta_d) &\approx \frac{1}{k}\sum_{n=1}^{k} \mathbb{E}(\Delta(b))_{b\in R_n(b_i)}\cdot p_k(n) \\
%		&= \frac{1}{k}\left(\mathbb{E}(\Delta(b))_{b\in R_1(b_i)}\cdot p_k(1)\right) + \frac{1}{k}\left(\sum_{n=2}^{k} \mathbb{E}(\Delta(b))_{b\in R_n(b_i)}\cdot p_k(n)\right) \\
%		\intertext{
%		Using Lemma \ref{lemma:clustering} and Remark \ref{rem:diminishing-values}, we know that $p_k(n)$ is diminishing as $n$ approaches $k$. This means that we can further approximate the expectation as
%		}
%		&\approx \frac{1}{k}\left(\mathbb{E}(\Delta(b))_{b\in R_1(b_i)}\cdot p_k(1)\right) + \epsilon
%	\end{align*}
%	We also note that
%	\begin{equation}
%	\label{eq:expected-delta}
%		\mathbb{E}(\Delta(b))=\sum_{n=1} \left(\mathbb{E}(\Delta(b))_{b\in R_n(b_i)}\cdot \frac{|R_n|}{|V|}\right).
%	\end{equation}
%	This means that $\mathbb{E}(\Delta(b))$ represents the average over the distribution of individual $\mathbb{E}(\Delta(b))_{b\in R_n(b_i)}$. Note that $\mathbb{E}(\Delta(b))\approx \frac{1}{k}\mathbb{E}(\Delta_d)\not\sim \mathbb{E}(\mathsf{Rep}_\Delta)$ is not proportional\footnote{In words, this states that $\mathbb{E}(\Delta(b))$, the expected proportion of minority voters over the whole graph is approximately $\frac{1}{k}\mathbb{E}(\Delta_d)$, the expected proportion of minority voters in a given district $d$, which however is \emph{not} proportional to the expected representation won. }
%	 (earlier, we detailed the non-proportionality of districting). Instead, the optimal strategy for any given party is to 'crack' the vote such that the opposing party wastes the most votes \cite{Bernstein2017AGap}. This means that the strategy for the majority and the minority party are different. 
%	
%	\noindent For the minority, this means that the optimal strategy is to maximize $\frac{1}{k}\mathbb{E}(\Delta_d)$ such that $\frac{1}{k}\mathbb{E}(\Delta_d) > 0.5$. This allows the minority to win the district with higher probability, causing the majority to waste more votes on average.\footnote{This discrepancy comes from the fact that nearer blocks are more likely appear, so we want to maximize this discrepancy in order to maximize $\frac{1}{k}\mathbb{E}(\Delta_d)$, as $\mathbb{E}(\Delta(b))$ is constant over the whole graph. }
%	 This means that the minority optimizes $\mathbb{E}(\Delta(b))_{b\in R_1(b_i)}$, the expected number of tiles adjacent to $b_i$. This minimizes $\epsilon$ by Equation \ref{eq:expected-delta}. Noting that $\mathbb{E}(\Delta(b))_{b\in R_1(b_i)}\sim \mathsf{ClusP}(\Delta)$ if we sample all $b_i\in V$ from our graph (they are the same measure---the similarity of adjacent tiles), this gives the desired conclusion that $\mathbb{E}(\mathsf{Rep}_\Delta)$ increases with $\mathsf{ClusP}(\Delta)$ for a minority. 
%	\end{proof}
%	
%	\begin{Rem}
%	We can extend the above conclusion for the majority. The majority already has $\mathbb{E}(\Delta(b))\approx \frac{1}{k}\mathbb{E}(\Delta_d)>0.5$. Then, the optimal strategy is to minimize $\frac{1}{k}\mathbb{E}(\Delta_d)$ to just above $0.5$ in order to crack a district $d$. Following a similar argument as above, we find that minimizing $\frac{1}{k}\mathbb{E}(\Delta_d)$ (and as a result, maximizing $\mathbb{E}(\mathsf{Rep}_\Delta)$) requires minimizing $\mathbb{E}(\Delta(b))_{b\in R_1(b_i)}$, which gives a negative correlation between $\mathsf{ClusP}(\Delta)$ and $\mathbb{E}(\mathsf{Rep}_\Delta)$ for a majority. 
%	\end{Rem}
